Human Side of Smart Contract Fuzzing: An Empirical Study

Smart contract (SC) fuzzing is a critical technique for detecting vulnerabilities in blockchain applications. However, its adoption remains challenging for practitioners due to fundamental differences between SCs and traditional software systems. In this study, we investigate the challenges practitioners face when adopting SC fuzzing tools by conducting an inductive content analysis of 381 GitHub issues from two widely used SC fuzzers: Echidna and Foundry. Furthermore, we conducted a user study to examine how these challenges affect different practitioner groups, SC developers, and traditional software security professionals, and identify strategies practitioners use to overcome them. We systematically categorize these challenges into a taxonomy based on their nature and occurrence within the SC fuzzing workflow. Our findings reveal domain-specific ease-of-use and usefulness challenges, including technical issues with blockchain emulation, and human issues with a lack of accessible documentation and process automation. Our results provide actionable insights for tool developers and researchers, guiding future improvements in SC fuzzer tool design.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> practice.tex <==
\begin{enumerate}[leftmargin=*, label=\textbf{\arabic*.}]
    \item \textbf{Usefulness}
    \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic*.}]
        \item \textbf{Reliability (Bug / Crash / Third-party)}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{Chain State Management Issues} – Failures related to managing blockchain state during testing, including forking inconsistencies, state variable manipulation problems, unexpected state leakage between tests, and challenges with storage layout resolution.
            \item \textbf{Dependency Conflicts} – Issues due to mismatches in Solidity versions, Ethereum clients, or linked libraries. Challenges related to external dependencies, including library version conflicts, failures in third-party components (like REVM), compiler compatibility issues, and dependency resolution failures in build systems.
            \item \textbf{Cross-Chain Compatibility Problems} – Difficulties when fuzzing contracts on different blockchain networks due to EVM implementation differences, varying RPC interfaces, and chain-specific behaviors that cause fork testing failures on non-Ethereum chains.
            \item \textbf{Cheatcode and VM Manipulation Problems} – Chain state setup primitives cause fuzzer crash, including timestamp manipulation incompatibilities, chain forking problems, cryptographic signing failures, and RPC call issues.
            \item \textbf{Unstable CI/CD Integration} – Fuzzers do not run smoothly in automated pipelines, making it hard to integrate into CI/CD workflows.
            \item \textbf{Unexpected Crash During Execution} – Runtime crashes, memory leaks, panics, and other execution failures that interrupt the fuzzing process and prevent complete test execution, including segmentation faults and resource exhaustion problems.
            \item \textbf{Environment Compatibility Issues} – Failures in building across different environments (Docker/NIX), and with tools behaving differently across operating systems, including segmentation faults on specific macOS versions and tests that pass on macOS but fail on Ubuntu.
            \item \textbf{Input Generation Failures} – Issues with generating valid test inputs, including type boundary violations, malformed calldata synthesis, limitations in handling constructor arguments, and failures in dictionary-based mutation strategies.
            \item \textbf{Configuration and Feature Interaction Issues} – Problems arising from conflicting configuration options, unexpected behavior when combining features, improper setting validation, and configuration parameters not being respected during execution.
            \item \textbf{Oracle Implementation Bugs} – Failures in the mechanisms that determine test outcomes, including assertion errors, false positives, incorrect error reporting, and oracle incompatibilities with state changes during test execution.
            \item \textbf{File and Cache Management Issues} – Problems with handling files and caches during fuzzing, including file locking issues in parallel execution, cache invalidation failures, directory structure errors, and artifact management challenges.
        \end{enumerate}

        \item \textbf{Consistency}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{State Management Inconsistencies} – Problems with blockchain state handling during test execution, including race conditions causing false negatives, state leakage between test functions, and inconsistent state between handler and invariant contexts.
            \item \textbf{Test Cases Not Replayable} – Inability to consistently replay previously discovered bugs or execute the same fuzzing campaign with identical results, including issues with corpus replay when contracts change and non-deterministic execution across different runs.
            \item \textbf{Non-Deterministic Behavior} – Execution outcomes that vary based on the environment, including differing gas measurements between CI and local environments, platform-specific behavior variations, and inconsistent compilation outputs across systems.
            \item \textbf{Discrepancy Within Output} – Issues with how fuzzing results are reported, including discrepancies between execution traces and reported outcomes, inconsistent gas reporting, and confusing or incomplete output formats that hinder result interpretation.
            \item \textbf{Lack of Credible Benchmark} – Difficulties in establishing fair and consistent benchmarks to compare different fuzzing tools, including lack of standardized test contracts, metrics, and methodologies for performance evaluation.
        \end{enumerate}

        \item \textbf{Performance (Speed / Coverage) \& Overhead (Memory / Storage)}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{High Gas Consumption} – Fuzzing generates transactions that exceed gas limits, leading to test failures.
            \item \textbf{Slow Execution Due to EVM Constraints} – Slow test execution due to inefficient EVM implementation, excessive transaction processing overhead, and poor utilization of available computational resources, including suboptimal thread usage and serialized execution paths.
            \item \textbf{On-Chain Data Access Inefficiencies} – Performance degradation when fuzzing contracts that interact with on-chain data, including slow slot fetching, excessive RPC calls, poor caching mechanisms, and bandwidth limitations when retrieving blockchain state.
            \item \textbf{Poor Path Exploration} – Fuzzer struggles to explore deep execution paths due to state-dependent logic or inefficient constraint solving. Difficulties in achieving comprehensive code coverage, including poor path exploration for complex conditions, inability to reach deep execution states, and challenges in handling state-dependent logic.
            \item \textbf{Input Generation and Mutation Inefficiencies} – Suboptimal test case generation strategies, including redundant input creation, poor coverage of value ranges, inadequate handling of complex input types, and ineffective dictionary management.
            \item \textbf{Inefficient Resource Utilization} – Fuzzers do not make optimal use of CPU/GPU resources during execution. Issues with effectively distributing computational resources across different test functions, handling varying test complexity, and optimizing fuzzing campaigns based on input characteristics.
            \item \textbf{Memory Management Issues} – Excessive memory consumption during fuzzing campaigns, including unbounded growth for long test sequences, memory leaks with complex contracts, and inefficient state representation leading to out-of-memory errors.
            \item \textbf{Storage and Disk Utilization Problems} – Challenges related to disk space usage, including excessive temporary file generation, inefficient corpus storage, and unnecessary artifact retention during fuzzing campaigns.
            \item \textbf{Debug and Tracing Overhead} – Performance penalties when enabling debugging features, trace collection, or coverage reporting, making it difficult to simultaneously debug and maintain reasonable execution speed.
        \end{enumerate}

        \item \textbf{Essential Feature (Support User Scenario)}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{Execution Control and Flow Management} – Insufficient control over test execution, including lack of timeout configuration, inability to continue testing after finding failures, missing support for gas and execution time limits, and poor handling of infinite loops or hanging test cases.
            \item \textbf{Limited On-Chain Oracles} – Users have limited options to test on-chain events.
            \item \textbf{Missing Hooks for Complex Contracts} – No support for pre/post-test conditions needed for real-world DeFi contracts.
            \item \textbf{Inadequate Multi-Contract Interaction} – Gaps in handling complex contract interactions, including limited support for delegatecall in fallback functions, poor handling of external libraries, incompatibility with proxy patterns, and challenges with multi-contract testing scenarios.
            \item \textbf{Limited Cross-Platform \& Cross-Chain Compatibility} – Missing support for various development environments and platforms, including incompatibility with Windows, limited support for monorepo structures, and limited support for cross-chain testing.
            \item \textbf{Blockchain State Manipulation Constraints} – Limited capabilities for setting up and controlling blockchain state during testing, including inadequate ETH balance management, insufficient support for state preservation across test runs, and missing primitives for manipulating chain parameters.
        \end{enumerate}
    \end{enumerate}

    \item \textbf{Ease-of-Use}
    \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic*.}]
        \item \textbf{Quality of Life Feature – Flexibility and Efficiency of Use}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{Fine-Grained Configuration Options} - Difficulty configuring fuzzer parameters globally or at granular levels (per-test, per-contract), including run counts, seed formats, and test behavior options.
            \item \textbf{Fine-Grained Input Generation and Constraint Strategies} - More mechanisms for bounding inputs, specifying value ranges, handling fixtures, and incorporating values from production environments.
            \item \textbf{Execution Control Deficiencies} - Lack of fine-grained control over test execution, including handling reverts, managing specific failures, and controlling test flow.
            \item \textbf{Preload Blockchain State} – Preload contract states from mainnet/testnet snapshots to save fuzzer runtime.
        \end{enumerate}

        \item \textbf{Quality of Life Feature – Error Prevention}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{Automate/Simplify Test Harness} - Difficulty in separating test functionality from contract code, testing multi-user scenarios, and creating specialized test environments.
            \item \textbf{Simplify Defining Target Functions} – Users struggle to specify which contract functions to fuzz.
            \item \textbf{Automatic Generation of Test Suite} - Limited export capabilities for test results, insufficient gas reporting for fuzz tests, and challenges in generating regression tests from failures.
        \end{enumerate}

        \item \textbf{Interpretability – Help Users Recognize, Diagnose, and Recover from Errors}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{Inadequate Non-Crash Failure Reporting} - Unclear, misleading, or absent error messages when contract deployment fails, functions revert or test case fails.
            \item \textbf{Unhelpful Crash Reporting} - Poor handling of arithmetic errors, unexpected opcodes, compilation issues, and other crash scenarios with insufficient debug information.
        \end{enumerate}

        \item \textbf{Interpretability – Visibility of System Status}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{Insufficient Performance Diagnostics} - Limited visibility into resource utilization, workload distribution, and runtime performance bottlenecks during fuzzing.
            \item \textbf{Limited Execution Tracing} - Missing, incomplete, or poorly formatted execution traces, particularly for failed test cases, successful fuzzing runs, and handler function failures. Inaccurate run counts, inadequate progress indicators, and limited status updates during fuzzing campaigns.
        \end{enumerate}

        \item \textbf{Interpretability – Recognition Rather than Recall}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{Lack of Visualization In Bug Report} - Lack of comprehensive reporting capabilities, including HTML reports, coverage visualization, progress indicators, and detailed failure information. Addresses not displayed in checksum format, and JSON output missing critical fields.
        \end{enumerate}

        \item \textbf{Learnability \& Documentation – Consistency and Standards}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{Hard-to-Configure Fuzzing Parameters} – Confusing or unintuitive configuration formats and undocumented configuration options. For example, Foundry provides no guidance on mutation depth, seed inputs, or transaction limits, but users are expected to understand their purpose and set them on a case-by-case basis. JSON/YAML configurations are not well-documented or too rigid.
            \item \textbf{Undocumented Behaviors and Side Effects} - Critical fuzzer behaviors not explicitly documented, including runtime contract deployment behavior, prank cheatcode effects, service contract addresses, and test case minimization logic.
            \item \textbf{Conceptual Model Misalignment} - Terminology and design choices that cause user confusion, including the dichotomy between different fuzzing approaches, unclear test patterns, and counterintuitive keywords.
        \end{enumerate}

        \item \textbf{Learnability \& Documentation – Help and Documentation}
        \begin{enumerate}[leftmargin=*, label=\textbf{\arabic{enumi}.\arabic{enumii}.\arabic*.}]
            \item \textbf{Poor Examples for Complex Use Cases} – Lack of comprehensive examples showcasing fuzzer features, particularly for complex scenarios like multi-user testing, constructor fuzzing, and edge case detection.
            \item \textbf{No Documented Best Practices} – Lack of recommended strategies for SC fuzzing. Limited guidance on effective debugging strategies, error interpretation, and test case reproduction for fuzzing issues. Critical steps in fuzzing workflow not explicitly documented.
            \item \textbf{No Fuzzing Resources Provided In Documentation} - Users who do not understand the basic premise of fuzzing, and fuzzing workflow have no way to learn the mental model required to work with SC fuzzers. And documentation of SC fuzzers provide no resource or links for users to educate themselves.
        \end{enumerate}
    \end{enumerate}
\end{enumerate}

\begin{table}[h]
\centering
\small % Reduce font size for compactness
\setlength{\tabcolsep}{2pt} % Reduce column padding
\resizebox{\textwidth}{!}{ % Scale table to text width
   \begin{tabular}{p{1.5cm}p{1.5cm}p{3cm}p{5cm}}
\toprule
\textbf{Level 1} & \textbf{Level 2} & \textbf{Level 3} & \textbf{Description} \\
\midrule
\textbf{Usefulness} & \textbf{Reliability} & Chain State Management Issues & Failures related to managing blockchain state during testing, including forking inconsistencies, state variable manipulation problems, and unexpected state leakage between tests. \\
& & Dependency Conflicts & Issues due to mismatches in Solidity versions, Ethereum clients, or linked libraries, including library version conflicts and compiler compatibility issues. \\
& & Cross-Chain Compatibility Problems & Difficulties when fuzzing contracts on different blockchain networks due to EVM implementation differences and chain-specific behaviors. \\
& & Cheatcode and VM Manipulation Problems & Chain state setup primitives cause fuzzer crashes, including timestamp manipulation incompatibilities and cryptographic signing failures. \\
& & Unstable CI/CD Integration & Fuzzers do not run smoothly in automated pipelines, making it hard to integrate into CI/CD workflows. \\
& & Unexpected Crash During Execution & Runtime crashes, memory leaks, panics, and other execution failures that interrupt the fuzzing process. \\
& & Environment Compatibility Issues & Failures in building across different environments (Docker/NIX), with tools behaving differently across operating systems. \\
& & Input Generation Failures & Issues with generating valid test inputs, including type boundary violations and malformed calldata synthesis. \\
& & Configuration and Feature Interaction Issues & Problems arising from conflicting configuration options and unexpected behavior when combining features. \\
& & Oracle Implementation Bugs & Failures in the mechanisms that determine test outcomes, including assertion errors and false positives. \\
& & File and Cache Management Issues & Problems with handling files and caches during fuzzing, including file locking issues and cache invalidation failures. \\
\cmidrule(lr){2-4}
& \textbf{Consistency} & State Management Inconsistencies & Problems with blockchain state handling during test execution, including race conditions and state leakage between test functions. \\
& & Test Cases Not Replayable & Inability to consistently replay previously discovered bugs or execute the same fuzzing campaign with identical results. \\
& & Non-Deterministic Behavior & Execution outcomes that vary based on the environment, including differing gas measurements between CI and local environments. \\
& & Discrepancy Within Output & Issues with how fuzzing results are reported, including discrepancies between execution traces and reported outcomes. \\
& & Lack of Credible Benchmark & Difficulties in establishing fair and consistent benchmarks to compare different fuzzing tools. \\
\cmidrule(lr){2-4}
& \textbf{Performance \& Overhead} & High Gas Consumption & Fuzzing generates transactions that exceed gas limits, leading to test failures. \\
& & Slow Execution Due to EVM Constraints & Slow test execution due to inefficient EVM implementation and excessive transaction processing overhead. \\
& & On-Chain Data Access Inefficiencies & Performance degradation when fuzzing contracts that interact with on-chain data, including slow slot fetching and excessive RPC calls. \\
& & Poor Path Exploration & Fuzzer struggles to explore deep execution paths due to state-dependent logic or inefficient constraint solving. \\
& & Input Generation and Mutation Inefficiencies & Suboptimal test case generation strategies, including redundant input creation and poor coverage of value ranges. \\
& & Inefficient Resource Utilization & Fuzzers do not make optimal use of CPU/GPU resources during execution. \\
& & Memory Management Issues & Excessive memory consumption during fuzzing campaigns, including unbounded growth for long test sequences. \\
& & Storage and Disk Utilization Problems & Challenges related to disk space usage, including excessive temporary file generation and inefficient corpus storage. \\
& & Debug and Tracing Overhead & Performance penalties when enabling debugging features, trace collection, or coverage reporting. \\
\cmidrule(lr){2-4}
& \textbf{Essential Feature} & Execution Control and Flow Management & Insufficient control over test execution, including lack of timeout configuration and inability to continue testing after finding failures. \\
& & Limited On-Chain Oracles & Users have limited options to test on-chain events. \\
& & Missing Hooks for Complex Contracts & No support for pre/post-test conditions needed for real-world DeFi contracts. \\
& & Inadequate Multi-Contract Interaction & Gaps in handling complex contract interactions, including limited support for delegatecall in fallback functions. \\
& & Limited Cross-Platform \& Cross-Chain Compatibility & Missing support for various development environments and platforms, including incompatibility with Windows. \\
& & Blockchain State Manipulation Constraints & Limited capabilities for setting up and controlling blockchain state during testing. \\
\midrule
\textbf{Ease-of-Use} & \textbf{Quality of Life Features} & Fine-Grained Configuration Options & Difficulty configuring fuzzer parameters globally or at granular levels. \\
& & Fine-Grained Input Generation and Constraint Strategies & More mechanisms for bounding inputs, specifying value ranges, and handling fixtures. \\
& & Execution Control Deficiencies & Lack of fine-grained control over test execution, including handling reverts and managing specific failures. \\
& & Preload Blockchain State & Preload contract states from mainnet/testnet snapshots to save fuzzer runtime. \\
\cmidrule(lr){2-4}
& \textbf{Interpretability} & Inadequate Non-Crash Failure Reporting & Unclear, misleading, or absent error messages when contract deployment fails. \\
& & Unhelpful Crash Reporting & Poor handling of arithmetic errors, unexpected opcodes, and compilation issues. \\
& & Insufficient Performance Diagnostics & Limited visibility into resource utilization and runtime performance bottlenecks. \\
& & Limited Execution Tracing & Missing, incomplete, or poorly formatted execution traces for failed test cases. \\
& & Lack of Visualization in Bug Report & Lack of comprehensive reporting capabilities, including HTML reports and coverage visualization. \\
\cmidrule(lr){2-4}
& \textbf{Learnability \& Documentation} & Hard-to-Configure Fuzzing Parameters & Confusing or unintuitive configuration formats and undocumented configuration options. \\
& & Undocumented Behaviors and Side Effects & Critical fuzzer behaviors not explicitly documented, including runtime contract deployment behavior. \\
& & Poor Examples for Complex Use Cases & Lack of comprehensive examples showcasing fuzzer features for complex scenarios. \\
& & No Documented Best Practices & Lack of recommended strategies for smart contract fuzzing. \\
& & No Fuzzing Resources Provided in Documentation & Users have no way to learn the mental model required to work with smart contract fuzzers. \\
\bottomrule
\end{tabular}
}
\caption{Taxonomy of Challenges in Smart Contract Fuzzing}
\label{tab:taxonomy}
\end{table}

==> result.tex <==
\subsection{Challenge Taxonomy} 
The complete taxonomy is presented in Table~[\ref{tab:taxonomy}] in the appendix. Here, we focus only on the subset of challenges that are specifically relevant to smart contract (SC) fuzzers.

\subsubsection{Sub-RQ1: Domain-Specific Usefulness / Usability Challenges in SC Fuzzing}
SC fuzzing introduces unique challenges not observed in traditional software fuzzing, primarily due to the stateful execution model of blockchains, constraints imposed by the EVM, gas usage limitations, and complex multi-contract interactions. These challenges reflect fundamental differences between SCs and conventional software systems. Drawing from our derived taxonomy [\ref{tab:taxonomy}], we identify and categorize the key domain-specific challenges as follows:

\begin{enumerate}
    \item \textit{Compiler Dependency and Cross-Chain Compatibility Issues}. Users reported significant technical reliability issues with Solidity language dependency conflicts. Solidity, the primary script language for SCs, was developed during the formative years of SC technology. It has gone through many breaking updates to accommodate for new features and patch language-level security flaws\cite{SolidityReleases}. Issues report Foundry's built-in compilation automation failing on code bases that contain multiple Solidity versions, or the internal Ethereum Virtual Machine (EVM) executor failing to accommodate binaries compiled from older Solidity versions. This problem is much less obvious in more stable languages like C and C++. In addition to issues with Solidity itself, different EVM-based chains like Ethereum, Polygon, and BSC have subtle differences that can break the fuzzer implementation, even though both Foundry and Echidna commit to supporting full-function cross-chain fuzzing. 
    
    For instance, one user reported that an invariant fork test on BSC failed due to a deserialization error when fetching an account. The issue appeared to stem from the use of 'unwrap' or 'expect', which panic on failure. Notably, the same code passed all local unit tests but failed only in the forked test environment, highlighting the complexity of cross-chain compatibility \cite{cross-chain}.
    
    \item \textit{EVM and Gas Constraints}. SCs operate under strict gas limits, causing fuzzing tests to fail if they exceed these limits. This differs fundamentally from traditional fuzzing, where execution cost is typically negligible. Furthermore, EVM emulation is computationally expensive compared to native execution, resulting in slower overall testing performance.
    For instance, one user reported encountering infinite loops in some fuzzing branches which causes the entire fuzzer to hang indefinitely. A user suggests adding `vm.callTimeout` and `vm.setGas` for improved gas control, allowing developers to set a timeout and adjust gas limit during contract calls \cite{gas-limit}.
    
    \item \textit{State Management Issues}. The stateful nature of SCs introduces technical issues with managing the chain state, including storage, balances, and other on-chain data. This requires fuzzers to correctly implement chain forking, state rollbacks, and storage slot resolution. Users reported blockchain state leaking between tests or running on corrupt states, causing inconsistent behavior\cite{state1, state2}. While traditional programs could be trusted to produce the same output given the same input, state variations and gas fluctuations make reproducing test cases more flaky for SCs. In addition, SCs fuzzers support on-chain fuzzing that interacts with blockchain state in real time. Fetching blockchain state through RPC calls is considerably slower compared to traditional fuzzing where all data is locally available. Fuzzers must also handle the preloading of blockchain state, including snapshotting and restoring state—processes that are unnecessary in traditional fuzzing environments, introducing issues with storage overhead.
    
    \item \textit{Lack of SC-Specific Documentations}. While there are plenty of online tutorials for popular program fuzzers, several users have reported difficulty finding tutorials and concrete examples of projects running SC fuzzers. Foundry documentation only provides incomplete code snippets, and users have reported difficulty extending the documentation to inform more complex real-world projects \cite{docum1, docum2}. Users have also reported confusion arising from missing documentation for SC-specific configuration options, as well as inconsistent terminology for critical features (e.g. referring to stateless fuzz testing as "fuzzing" while stateful fuzz testing as "invariant testing")\cite{docum3}.
    
    \item \textit{Manual Yet Inflexible Fuzzer Setup Process}. Users have complained of the lack of basic automation in fuzzer setup \cite{config1}. While an effective fuzz driver could be simply generated as a wrapper around the target contract's functions-under-test, Foundry and Echidna have not introduced any utility feature to enable it. Some community members have resorted to starting "fuzz-utils", a separate automation tool for Echidna\cite{crytic2023fuzzutils}. Moreover, the lack of automation is not rewarded in a high level of customizability in the fuzzing process. Users do not have control over per-test timeouts, max executions per function, or continuous fuzzing after the initial crash. Advanced users also requested for more modular accommodation for custom path resolution mechanisms like SMT solvers, which is not met.
\end{enumerate}

Addressing these challenges requires \textbf{specialized fuzzing techniques}, including \textbf{state snapshotting, differential execution, gas-aware fuzzing, and structured input generation}, which are not necessary for traditional software fuzzing.
All of the findings from the "Ease-of-use" category can be generalized for all of the fuzzing tools.

\subsection{Outcome of User Study}
In the following, we present our observations from analyzing the user studies conducted with SC developers and fuzzing practitioners. Our qualitative findings analyze the challenges perceived by both groups and their attitude toward future adoption (Sub-RQ2), how these challenges manifest across different practitioner backgrounds, and the strategies used to overcome them (Sub-RQ3) [\ref{RQ:Sub-RQ2}].

\subsubsection*{Summary of Key Findings}
Our study revealed several critical challenges facing practitioners when adopting SC fuzzing tools:
\begin{enumerate}
    \item \textbf{Documentation and Knowledge Gap}: Both practitioner groups struggled with insufficient documentation, though SC developers were more severely impacted
    \item \textbf{Mental Model Misalignment}: SC developers conceptualized fuzzing differently than how SC fuzzers are implemented
    \item \textbf{Technical Jargon}: Unexplained terminology created barriers, particularly for SC developers
    \item \textbf{Tool Interpretability}: Error messages and feedback from the fuzzing tools often led to confusion
    \item \textbf{Domain Knowledge Advantage}: SC developers leveraged their domain expertise in certain aspects despite technical challenges
\end{enumerate}

\subsubsection{Sub-RQ2: How Do Challenges Affect Practitioners And Any Difference Between Groups}
Our quantitative analysis measured user fuzz performance scores, self-reported satisfaction, and willingness to adopt technology based on post-study interviews. Due to the time limit of our user study, we only observed usability challenges affecting participants' performance.

The lack of SC fuzzer-specific documentations and code examples impact all participants, especially SC developers. For developers, we observed a significant gap between their mental models of fuzzing and SC fuzzers' actual implementation paradigm. SC developers conceptualize fuzzing as adding randomness to unit tests. While this mental model is helpful for learning stateless program fuzzers, SC fuzzers require more steps to set up, as shown in our task list. No step-by-step code example is provided in the Foundry documentation to bridge this knowledge gap. The challenge was compounded by inconsistent terminology and use of unexplained jargon. Developers particularly struggled to differentiate between ``invariant testing'' and ``fuzz testing,'' which were presented as separate techniques despite invariant testing being essentially fuzz testing with stateful sequence support. These conceptual confusions manifested in frustration and failure to follow best practice. This misconception led P1 and P3 to create test harnesses with hardcoded API sequences instead of defining flexible property boundaries that could be effectively fuzzed. Around the 30 minutes mark, both P2 and P3 abandoned attempts to conceptually understand the documentation altogether, instead relying on AI or themselves to write and debug the task.
\begin{quote}
      It's unclear to me where the randomness happens. Don't you need to add randomness somewhere? The documentation doesn't even mention the word "random". (P1)
      
      Documentation doesn't really help me here. It's too much. Fuzzing is not trivial. (P3)
\end{quote}

Moreover, the Foundry documentation uses jargon that are essential for fuzzing performance without explaining them with concrete examples. For example, 'ghost variables' are an essential feature in invariants that tracks expected values across fuzzing executions. But the term itself is obscure for users without a background in formal verification. While P1 and P4 (both PhD students with relevant training) understood and implemented this concept easily, SC developers P2 and P3 struggled with understanding or leveraging the feature. P2 managed to set up ghost variables with AI assistance, while P3 refused AI assistance and failed to implement correct invariants. Another example is the concept 'actor pattern', a Foundry-specific programming paradigm that enables the SC fuzzer to assume multiple roles in a single fuzzing campaign and simulate peer-to-peer communication. Since no code example is provided, none of our participants was able to understand or follow this guideline. Instead, they used the fuzz harness to interact with the target contract in a traditional client-server relationship. This approach, while sufficient for revealing individual bugs like \#2 or \#3, restricted the fuzz harness to testing only one specific bug at a time. This limitation became evident when P4 needed to completely rewrite the harness between testing for bug \#2 and bug \#3. Similarly, P2 abandoned the task due to fatigue after identifying bug \#3, unaware that finding bug \#2 would have required only a one-line code change had they properly implemented the actor pattern.

Fuzzing practitioners encountered fewer challenges following the documentation. P4 quickly recognized similarities between SC fuzzing and traditional program fuzzing paradigms, correctly identifying invariants as analogous to bug oracles and harnesses as similar to fuzz targets. But they recommended harness automation based on their expert experienced better tools in traditional program fuzzers.
\begin{quote}
Automating the fuzz harness generation would be a good idea. You could provide a harness that fuzzes all endpoints, and let us cut it down. That at least gives us something to start with. (P4)
\end{quote}

Invariant writing is the only step where SC developers performed better by leveraging domain insight, as the primary challenge in crafting effective invariants stemmed from participants' understanding of the contract's standard behavior. As P1 explained:
\begin{quote}
    I can see this contract follows the standard ERC-20 interface, so I know what conditions to assert. (P1)
\end{quote}
All three developers correctly chose to focus on testing the \texttt{deposit}, \texttt{withdraw}, and \texttt{withdrawAll} endpoints, with the experienced developer P3 identifying the crashing bug \#1 without even running the fuzzer. Fuzzing practitioners took a more analytical approach to API selection. P4 categorized target APIs into ``data sources'' and ``data sinks,'' correctly inferring which APIs needed to be tested in sequence from a dataflow perspective. This approach enabled P4 to identify the \texttt{deposit} function as an essential prerequisite for other endpoints and successfully target valid API sequences.

Lastly, our user study revealed some interpretability challenges not reported in the GitHub issues. First, when a user-defined invariant was false by default, Foundry displayed a generic ``failed to setup environment'' message rather than clearly indicating an invariant failure. Since this generic message also appears for other setup issues, participants struggled to determine whether the problem originated from their harness configuration or from the invariants themselves. For example, P4 created an invariant to verify that a user's balance should be greater than zero after deposit functions execute. This approach failed because Foundry checks invariants once before the first execution, when no deposits have occurred yet, leaving P4 confused about the source of the setup failure.

Second, Foundry only reports crashes when an invariant is violated. The fuzzer will report ``all tests passed'' even if every function call crashes, as long as no invariant is violated. This behavior directly hindered P1's progress: despite writing the correct invariant to reveal bug \#2, bug \#1 prevented sufficient coverage to trigger bug \#2. Only participants with exceptional attention to detail could identify this behavior without researcher intervention. When P4 encountered the same ``all tests passed'' message, he analyzed the fuzz statistics, noticed that zero calls had passed, and correctly deduced that the ``deposit'' API must be consistently crashing, prompting him to revise his invariants to test for bug \#1.

\subsubsection{Sub-RQ3: User Strategies to Overcome Challenge}
The participants in our study employed various strategies to overcome the documentation and usability challenges they encountered:

\begin{enumerate}
    \item \textbf{AI Assistance}: Less-experienced developers who leveraged AI assistants (P1, P2) gained better understanding of the documentation and generated working fuzz harnesses to at least run the fuzzer, while the more experienced developer P3 who did not use AI failed to run the fuzzer. P1 provided the AI with official Foundry documentation and requested workflow explanations specific to the task, while P2 described the scenario and target contract to generate starter code. Although AI-generated implementations contained some errors, they provided concrete starting points tailored to the specific context.

    \item \textbf{Mental Model Transfer}: Fuzzing experts experienced significantly fewer documentation challenges by mapping SC fuzzing concepts to familiar concepts from traditional fuzzing. P4's approach of categorizing APIs into ``data sources'' and ``data sinks'' demonstrates how transferring mental models from traditional software security can help overcome SC-specific challenges.

    \item \textbf{Domain Knowledge Application}: SC developers leveraged their understanding of smart contract standards and interfaces to determine what conditions to assert in invariants, even when struggling with the technical aspects of the fuzzing process.

    \item \textbf{Pragmatic Approach}: When facing comprehension obstacles, some participants (P2, P3) abandoned attempts to understand conceptually and switched to a more pragmatic, trial-and-error approach after approximately 30 minutes of effort.
\end{enumerate}

\begin{table}[h]
\centering
\caption{Mapping Challenges to Different Practitioner Groups}
\label{tab:practitioner-challenges}
\begin{tabular}{@{}p{3cm}|p{5cm}|p{5cm}@{}}
\toprule
\textbf{Challenge Type} & \textbf{SC Developers (Group A)} & \textbf{Fuzzing Practitioners (Group B)} \\
\midrule
Documentation Gaps & Severely impacted & Moderately impacted \\
\midrule
Mental Model Alignment & Major challenge (fuzzing $\neq$ randomized unit tests) & Minor challenge (recognized similarities to traditional fuzzing) \\
\midrule
Technical Jargon & Significant barrier (e.g., ``ghost variables'') & Less problematic (familiar with related concepts) \\
\midrule
Tool Interpretability & Struggled with error messages & Better at interpreting fuzzer behavior \\
\midrule
API Selection & Domain-based approach & Analytical data flow approach \\
\midrule
Invariant Writing & Leveraged domain knowledge effectively & Analytical approach, sometimes less effective \\
\bottomrule
\end{tabular}
\end{table}

\subsection{Connecting Domain-Specific Challenges with User Experiences}
\label{sec:connecting-challenges}

Our findings from Sub-RQ1 and Sub-RQ2 demonstrate a clear relationship between the domain-specific challenges inherent to SC fuzzing tools and the practical difficulties experienced by different practitioner groups. Table~\ref{tab:challenge-connections} maps these relationships.

\begin{table}[h]
\centering
\caption{Connections Between Domain-Specific Challenges and User Experiences}
\label{tab:challenge-connections}
\begin{tabular}{@{}p{4cm}|p{10cm}@{}}
\toprule
\textbf{Domain-Specific Challenge} & \textbf{Observed Impact on Practitioners} \\
\midrule
Lack of SC-Specific Documentation & SC developers struggled significantly with conceptual understanding, while fuzzing practitioners could partially compensate using mental models from traditional fuzzing \\
\midrule
Manual Yet Inflexible Fuzzer Setup & P4 specifically recommended harness automation based on experience with traditional fuzzers; All participants struggled with the lack of flexibility \\
\midrule
State Management Issues & Participants encountered confusing behavior with invariant checking and state persistence between tests \\
\midrule
Technical Jargon & Terms like ``ghost variables'' and ``actor pattern'' created barriers, especially for SC developers without formal verification background \\
\midrule
EVM and Gas Constraints & Not directly observed in our study due to time constraints, but potentially contributing to tool performance issues \\
\bottomrule
\end{tabular}
\end{table}

These connections illustrate how the fundamental technical challenges in SC fuzzing directly translate to usability barriers for practitioners. Notably, while both practitioner groups encountered these challenges, their different backgrounds and mental models led to varied experiences and coping strategies.

\begin{enumerate}
    \item \textit{Compiler Dependency and Cross-Chain Compatibility Issues}. Users reported significant technical reliability issues with Solidity language dependency conflicts. Solidity, the primary script language for SCs, was developed during the formative years of SC technology. It has gone through many breaking updates to accommodate for new features and patch language-level security flaws\cite{SolidityReleases}. Issues report Foundry's built-in compilation automation failing on code bases that contain multiple Solidity versions, or the internal Ethereum Virtual Machine (EVM) executor failing to accommodate binaries compiled from older Solidity versions. This problem is much less obvious in more stable languages like C and C++. In addition to issues with Solidity itself, different EVM-based chains like Ethereum, Polygon, and BSC have subtle differences that can break the fuzzer implementation, even though both Foundry and Echidna commit to supporting full-function cross-chain fuzzing. 
    
    For instance, one user reported that an invariant fork test on BSC failed due to a deserialization error when fetching an account. The issue appeared to stem from the use of 'unwrap' or 'expect', which panic on failure. Notably, the same code passed all local unit tests but failed only in the forked test environment, highlighting the complexity of cross-chain compatibility \cite{cross-chain}.
    % \item \textit{SC-Specific Features}. Fuzzers must implement cheatcodes (such as Foundry's \texttt{vm.prank}) that manipulate blockchain state, which have no equivalent in traditional fuzzing environments. There are also challenges with multi-contract interactions, as SCs frequently call other contracts, including proxies and those using delegatecall patterns. This necessitates complex inter-contract fuzzing logic. Additionally, while traditional fuzzers don't typically need oracles to verify correctness, SC fuzzers rely heavily on them to check blockchain state validity.
    \item \textit{EVM and Gas Constraints}. SCs operate under strict gas limits, causing fuzzing tests to fail if they exceed these limits. This differs fundamentally from traditional fuzzing, where execution cost is typically negligible. Furthermore, EVM emulation is computationally expensive compared to native execution, resulting in slower overall testing performance.
    For instance, one user reported encountering infinite loops in some fuzzing branches which causes the entire fuzzer to hang indefinitely. A user suggests adding `vm.callTimeout` and `vm.setGas` for improved gas control, allowing developers to set a timeout and adjust gas limit during contract calls \cite{gas-limit}.
    \item \textit{State Management Issues}. The stateful nature of SCs introduces technical issues with managing the chain state, including storage, balances, and other on-chain data. This requires fuzzers to correctly implement chain forking, state rollbacks, and storage slot resolution. Users reported blockchain state leaking between tests or running on corrupt states, causing inconsistent behavior\cite{state1, state2}. While traditional programs could be trusted to produce the same output given the same input, state variations and gas fluctuations make reproducing test cases more flaky for SCs. In addition, SCs fuzzers support on-chain fuzzing that interacts with blockchain state in real time. Fetching blockchain state through RPC calls is considerably slower compared to traditional fuzzing where all data is locally available. Fuzzers must also handle the preloading of blockchain state, including snapshotting and restoring state—processes that are unnecessary in traditional fuzzing environments, introducing issues with storage overhead.
    \item \textit{Lack of SC-Specific Documentations}. While there are plenty of online tutorials for popular program fuzzers, several users have reported difficulty finding tutorials and concrete examples of projects running SC fuzzers. Foundry documentation only provides incomplete code snippets, and users have reported difficulty extending the documentation to inform more complex real-world projects \cite{docum1, docum2}. Users have also reported confusion arising from missing documentation for SC-specific configuration options, as well as inconsistent terminology for critical features (e.g. referring to stateless fuzz testing as "fuzzing" while stateful fuzz testing as "invariant testing")\cite{docum3}.
    \item \textit{Manual Yet Inflexible Fuzzer Setup Process}. Users have complained of the lack of basic automation in fuzzer setup \cite{config1}. While an effective fuzz driver could be simply generated as a wrapper around the target contract's functions-under-test, Foundry and Echidna have not introduced any utility feature to enable it. Some community members have resorted to starting "fuzz-utils", a separate automation tool for Echidna\cite{crytic2023fuzzutils}. Moreover, the lack of automation is not rewarded in a high level of customizability in the fuzzing process. Users do not have control over per-test timeouts, max executions per function, or continuous fuzzing after the initial crash. Advanced users also requested for more modular accommodation for custom path resolution mechanisms like SMT solvers, which is not met.
    % \item \textit{Undocumented Runtime Behaviors}. Need user to explicitly exclude service contract addresses. How fuzzer scrape source code for input values that may conflict with preset exclusion logic. Fuzzer checks invariants once before first execution. 
\end{enumerate}
